PolyShard: Coded Sharding Achieves Linearly Scaling Efficiency and Security Simultaneously

Today's blockchain designs suffer from a trilemma claiming that no blockchain system can simultaneously achieve decentralization, security, and performance scalability. For current blockchain systems, as more nodes join the network, the efficiency of the system (computation, communication, and storage) stays constant at best. A leading idea for enabling blockchains to scale efficiency is the notion of sharding: different subsets of nodes handle different portions of the blockchain, thereby reducing the load for each individual node. However, existing sharding proposals achieve efficiency scaling by compromising on trust - corrupting the nodes in a given shard will lead to the permanent loss of the corresponding portion of data. In this paper, we settle the trilemma by demonstrating a new protocol for coded storage and computation in blockchains. In particular, we propose PolyShard: ``polynomially coded sharding'' scheme that achieves information-theoretic upper bounds on the efficiency of the storage, system throughput, as well as on trust, thus enabling a truly scalable system. We provide simulation results that numerically demonstrate the performance improvement over state of the arts, and the scalability of the PolyShard system. Finally, we discuss potential enhancements, and highlight practical considerations in building such a system.

==> ISIT/0-ISIT-abstract.tex.tex <==
\begin{abstract}
Today's blockchain designs suffer from a trilemma claiming that no blockchain system can simultaneously achieve decentralization, security, and performance scalability. For current blockchain systems, as more nodes join the network, the efficiency of the system (computation, communication, and storage) stays constant at best. A leading idea for enabling blockchains to scale efficiency is the notion of sharding: different subsets of nodes handle different portions of the blockchain, thereby reducing the load for each individual node. However, existing sharding proposals achieve efficiency scaling by compromising on trust - corrupting the nodes in a given shard will lead to the permanent loss of the corresponding portion of data. In this paper, we settle the trilemma by demonstrating a new protocol for coded storage and computation in blockchains. In particular, we propose  {\tt PolyShard}: ``polynomially coded sharding'' scheme that achieves information-theoretic upper bounds on the efficiency of the storage, system throughput, as well as on trust, thus enabling a truly scalable system. %We provide simulation results that numerically demonstrate the performance improvement over state of the arts, and the scalability of the {\tt PolyShard} system. Finally, we discuss potential enhancements, and highlight practical considerations in building such a system.
% Today's blockchains do not scale in a meaningful sense. As more nodes join the system, the efficiency of the system (computation, communication, and storage) degrades, or at best stays constant. A leading idea for enabling blockchains to scale efficiency is the notion of sharding: different subsets of nodes handle different portions of the blockchain, thereby reducing the load for each individual node. However, existing sharding proposals achieve efficiency scaling by compromising on trust - corrupting the nodes in a given shard will lead to the permanent loss of the corresponding portion of data. We observe that sharding is similar to replication coding, which is known to be inefficient and fragile in the coding theory community. In this paper, we demonstrate a new protocol for coded storage and computation in blockchains. In particular, we propose  {\tt PolyShard}: ``polynomially coded sharding'' scheme that achieves information-theoretic upper bounds on the efficiency of the storage, system throughput, as well as on trust, thus enabling a truly scalable system. We provide simulation results that numerically demonstrate the performance improvement over state of the arts, and the scalability of the {\tt PolyShard} system. Finally, we discuss potential enhancements, and highlight practical considerations in building such a system.
\end{abstract}
%\textit{A full version of this paper is accessible at} \cite{}.

==> ISIT/1-ISIT-intro.tex <==
\section{Introduction}\label{sec:intro}
While Blockchain systems promise a host of new and exciting applications, such as digital cryptocurrency~\cite{nakamoto2008bitcoin}, industrial IoT~\cite{bahga2016blockchain}, and healthcare management~\cite{mettler2016blockchain}, their scalability remains a critical challenge \cite{croman2016scaling}. In fact, a well-known blockchain trilemma has been raised~\cite{trilemma} claiming that no  decentralized ledger system can simultaneously achieve 1) security (against adversarial attacks), 2) decentralization (of computation and storage resources), and 3) scalability (of throughput with the network size). All existing major blockchains either achieve decentralization at the cost of efficiency, or efficiency at the cost of decentralization and/or security.



The focus of this paper is to formalize and study a version of the blockchain trilemma, in order to understand whether it is fundamental to blockchain systems. Corresponding to the three traits in the trilemma, we study the following performances measures of blockchain systems: security - measured as the number of malicious nodes the system can tolerate,   decentralization - measured as the fraction of the block chain (or ledger) that is stored and processed by each node (we denote its inverse by {\em storage efficiency}), and scalability - measured as the total \emph{throughput} of the system that is the number of computations performed in the system (e.g., number of transactions verified) in a unit period of time.

%The focus of this paper is to study a version of the blockchain trilemma, and understand whether it is fundamental to blockchain systems. Corresponding to the three traits in the trilemma, we study the following performances measures of blockchain systems: \emph{security} - measured as the number of malicious nodes the system can tolerate,  {\em storage efficiency} - measured as the maximum size of the blockchain that can be handled by nodes with fixed storage sizes, and {\em throughput} - measured as the number of computations performed (e.g., number of transactions verified) in a unit period of time.


% The scalability is with respect to three important performance metrics: the {\em throughput} - measured as the number of computations performed (e.g., number of transactions verified) in a distinct period of time, the {\em storage efficiency} - measured as the maximum size of the blockchain that can be handled by nodes with fixed storage sizes, and the \emph{security} - measured as the number of malicious nodes the system can tolerate.  By scalable, we mean that all these three metrics should  improve as $N$ increases, namely, all-round scalability.

% Blockchain systems maintain a distributed trusted ledger and can do finite-state computations. They can execute a wide range of programs in a trust-free setting, and has promised a host of new and exciting applications in various areas including digital cryptocurrency~\cite{nakamoto2008bitcoin}, industrial IoT~\cite{bahga2016blockchain}, and healthcare management~\cite{mettler2016blockchain}. However, to enable these applications, we need blockchain systems that {\em scale well with the number $N$ of participating nodes} \cite{croman2016scaling}. The scalability is with respect to three important performance metrics: the {\em throughput} - measured as the number of computations performed (e.g., number of transactions verified) in a distinct period of time, the {\em storage efficiency} - measured as the maximum size of the blockchain that can be handled by nodes with fixed storage sizes, and the \emph{security} - measured as the number of malicious nodes the system can tolerate.  By scalable, we mean that all these three metrics should  improve as $N$ increases, namely, all-round scalability.

% All-round scalability is a remarkably high expectation and has been one of the greatest challenges faced by 
Within this context, let's examine the current blockchain systems. %The system performance are expected to not go worse (at best) as the number of nodes $N$ increases.
% Indeed, even state-of-the-art scaling solutions \cite{sompolinsky2015secure,eyal2016bitcoin,luu2016secure,kokoris2017omniledger,gencer2017short} expect performance metrics to not get worse (at best) as the number of nodes $N$ increases {\color{red} [By Fisher: You cited scaling solutions such as Omniledger. Does their performance go worse with increasing $N$ as Bitcoin?]}.
%\begin{figure}[t]
%\centering
 %   \includegraphics[width=0.5\linewidth]{trilemma.pdf}
  %  \caption{Blockchain trilemma. No current blockchain system can simultaneously achieve decentralization, security, and scalability.}
  %  \label{fig:trilemma}
  %  \vspace{-2mm}
%\end{figure}
Bitcoin~\cite{nakamoto2008bitcoin} and Ethereum~\cite{wood2014ethereum} are designed based on a {\em  full replication} system, where each network node  stores the entire blockchain and replicates all the computations (e.g., transaction verifications), as demonstrated in Figure \ref{fig:fr_and_sharding}(a). This feature enables  high security (of tolerating 49\% adversarial nodes), however drastically limits the storage efficiency and throughput of the system: they stay constant regardless of the number of nodes $N$. For example, Bitcoin restricts its block size to 1 MB, and processing rate to 7 transactions/sec~\cite{gervais2016security}. In practice, the computational burden even increases with $N$ (e.g., mining puzzles get harder as time progresses and more users join), causing the throughput to drop. 




%, inherently restricting the throughput. The main reason that hinders these conventional technologies from scaling is that their key underpinning storage and computation methods involve {\em  full replication}: Each network node  stores the entire blockchain and replicates all the computations (verifications), as demonstrated in Figure \ref{fig:fr_and_sharding}(a). This feature gives a full replication system  high security (of tolerating 49\% adversarial nodes).  But the storage efficiency and throughput of the system is compromised: They stay constant regardless of the number of nodes $N$. In practice, the computational burden even increases with $N$ (e.g., mining puzzles get harder as time progresses and more users participate), causing the throughput to drop.
% When a new node joins a blockchain system that is based on full replication, it stores the entire blockchain locally. For any incoming blocks of transactions, each node verifies them locally at its highest processing rate.

To scale out throughput and storage efficiency, the leading solution being discussed in the blockchain literature is via {\em sharding}  \cite{luu2016secure,kokoris2017omniledger,gencer2017short}. The key idea is to partition the blockchain into $K$ independent sub-chains, which are then replicated separately at $q=\frac{N}{K}$ nodes to yield $K$ smaller full-replication systems, a.k.a., shards (Figure \ref{fig:fr_and_sharding}(b)). This way, both storage efficiency and throughput are improved by a factor of $K$. However, to scale this improvement with network size, $K$ must increase linearly with $N$. Consequently, the number of nodes $q$ per shard has to be held constant, which allows an attacker to corrupt as few as $q/2$ nodes to compromise a shard. This yields a security level of $q/2$, which approaches zero as $N$ grows. Although various efforts have been made to alleviate this security issue (e.g., by periodically shuffling the nodes \cite{kokoris2017omniledger}), they are susceptible to powerful adversaries (e.g., who can corrupt the nodes {\em after} the shuffling), yet none scale security.

%they incur non-negligible system overhead, yet none achieves security scalability.
% ratio of adversarial nodes that can be tolerated becomes exceedingly small, i.e., the adversary should control strictly less than $\frac{q}{N}$ fraction of nodes, which approaches zero as $N$ becomes large. %Hence, sharding achieves linear scaling of throughput and storage efficiency at the cost of decreasing the security guarantees.

% Existing sharding schemes propose some methods to alleviate this security issue: for example, by choosing random nodes through a cryptographic primitive to participate in a given shard, and using methods of shard rotation \cite{kokoris2017omniledger}. However, a powerful adversary can easily take control of a given shard by corrupting the users {\em after they have been chosen to participate in the shard}. Moreover, when the nodes are not assumed to be honest, but only rational, it might be in the interest of the small number of nodes in a given shard to {\em collude} to get illegal gains. Thus, sharding in its present form trades off security for efficiency scaling.
\begin{figure}[t]
\vspace{-3mm}
\centering
    \subfloat[]{\includegraphics[width=0.3\linewidth]{figures/full_replication.png}}\hspace{10pt}
    \subfloat[]{\includegraphics[width=0.35\linewidth]{figures/sharding.png}}
    \caption{(a) Full replication: A blockchain system with 30 nodes, each of which is capable of verifying 3 transactions per epoch. 3 transactions verified per epoch. Can tolerate $\frac{N}{2}-1=14$ malicious nodes. (b) Sharding with 3 shards: With 3-sharding, the ledger is partitioned into 3 sub-ledgers, and transactions are limited to between the accounts within the same sub-ledger. 9 transactions verified per epoch. Can tolerate $\frac{N}{2K}-1=4$ malicious nodes. Sharding improves the storage and throughput efficiency by 3 time, at the cost of compromising security by about 3 times.}
    \label{fig:fr_and_sharding}
\end{figure}

In summary, both full replication and sharding based blockchain systems make trade-offs between the scalability of throughput, storage efficiency, and security. However, such a trade-off is far from optimal from information theoretical point of view. Given the $N\times$ computation and $N\times$ storage resources across all the $N$ network nodes, the following information-theoretic upper bounds hold: $\textup{security} \leq \Theta(N)$; $\textup{throughput} \leq \Theta(N)$; $\textup{storage efficiency} \leq \Theta(N)$.
% On the other hand, the information-theoretic bounds offer a drastically different view. These bounds are not specific to a method or technology. This independence lends them a fundamental value and are derived as follows.
% Suppose all computation and storage, currently distributed across $N$ network nodes, can be used in a centralized manner. This allows a total of $N\times$ computation and $N\times$ storage. Thus the following information-theoretic upper bounds holds for any decentralized technology:
% $$
% \textup{Information-theoretic upper bounds}: \quad \textup{throughput} \leq \Theta(N);   \quad  \textup{storage efficiency} \leq \Theta(N),
% $$
%\vspace{-1.5em}
% $$
% \textup{security} \leq \Theta(N); \quad \textup{throughput} \leq \Theta(N);   \quad  \textup{storage efficiency} \leq \Theta(N).
% $$
It is intuitive that these bounds can be \emph{simultaneously} achieved by a centralized system, allowing all the three metrics to scale. However, as pointed out by the trilemma, this has not been achieved by any existing decentralized system. This raises the following fundamental open problem: 
% At this point, we are interested in the question that whether such a security-scaling tradeoff is fundamental to decentralized blockchain payment systems or 

% We note that existing sharding schemes propose some methods to alleviate the security issue: for example, by choosing random nodes through a cryptographic primitive to participate in a given shard, and using methods of shard rotation \cite{kokoris2017omniledger}. However, a powerful adversary can easily take control of a given shard by corrupting the users {\em after they have been chosen to participate in the shard}. Moreover, when the nodes are not assumed to be honest, but only rational, it might be in the interest of the small number of nodes in a given shard to {\em collude} to get illegal gains. Thus, sharding in its present form trades off trust for throughput, i.e., the larger the $f$, the more the security whereas lesser the scaling of throughput and computational abilities of the block-chain payment system (which scale like $k = \frac{n}{f}$). An important question  is whether such a trust-scaling tradeoff is fundamental to decentralized blockchain payment systems or whether clever methodologies can achieve different scaling behaviors.
% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.6\textwidth]{scalingSecurity.pdf}
%   \caption{Comparison of block verification schemes.}
%   \label{fig:scaleSecure}
% \end{figure}

% \begin{tcolorbox}
% Is there a blockchain verification scheme that achieves the security of the full replication scheme and the scaling of the sharding scheme \emph{simultaneously}?
% \end{tcolorbox}

\begin{tcolorbox}[width = \columnwidth, bottom=1pt,top=1pt]
Is there a blockchain design that \emph{simultaneously} scales storage efficiency, security, and throughput?
\end{tcolorbox}
% We answer this question affirmatively, and propose a coded block verification scheme, named ``polynomially coded sharding'' ({\tt {\tt PolyShard}}) to achieve this goal.

We answer this question affirmatively by introducing the concept of {\em coded sharding}. In particular, we propose  {\tt PolyShard} (polynomially coded sharding), a scheme that simultaneously  achieves linear scaling in throughput, storage efficiency, and security (i.e., $\Theta(N)$). We show that {\tt Polyshard} achieves all three information-theoretic upper bounds and enables a truly scalable blockchain system. (see Table~\ref{table:compare})
% More precisely, in a system composed of $N$ nodes, we show that {\tt PolyShard} provides both scalability and adversarial protection capability, i.e., it is possible to get a factor $N$ increase in efficiency (throughput / storage), while {\em simultaneously} maintaining the adversarial protection also as $\Theta(N)$
\begin{table}[h]
\vspace{-1mm}
  \centering
  \scalebox{0.82}{
  \begin{tabular}{| c | c | c | c | }
    \hline
    \rule{0pt}{10pt} & Storage efficiency & Security & Throughput \\ \hline
    \rule{0pt}{10pt} Full replication & $O(1)$  & $\Theta(N)$  &  $O(1)$ \\ \hline
    \rule{0pt}{10pt}  Sharding & $\Theta(N)$ & $O(1)$  & $\Theta(N)$ \\ \hline
     \rule{0pt}{10pt} Information-theoretic limit & $\Theta(N)$  & $\Theta(N)$  & $\Theta(N)$ \\ \hline
     \rule{0pt}{10pt} {\tt PolyShard} (this paper) & $\Theta(N)$  & $\Theta(N)$  & $\Theta(N)$ \\ \hline
  \end{tabular}
  }
  \caption{Performance comparison of the proposed {\tt PolyShard} verification scheme with other benchmarks and the information-theoretic limits.}\label{table:compare}
\end{table}

{\tt PolyShard} is inspired by recent developments in \emph{coded computing}~\cite{LMA_all,li2016fundamental,lee2018speeding,LMA16_unify,dutta2016short,yu2017polynomial,karakus2017straggler,TLDK-ICML,yu2018lagrangeNIPS}, in particular Lagrange Coded Computing~\cite{yu2018lagrangeNIPS}, which provides a transformative framework for injecting computation redundancy in unorthodox coded forms in order to deal with failures and errors in distributed computing. The key idea behind {\tt PolyShard} is that instead of storing and processing a single uncoded shard as done conventionally, each node stores and computes on a coded shard of the same size that is generated by linearly mixing uncoded shards (Figure \ref{fig:polyshard}), using the well-known Lagrange polynomial. This coding provides computation redundancy to simultaneously provide security against erroneous results from malicious nodes, which is enabled by noisy polynomial interpolation techniques (e.g., Reed-Solomon decoding).

% \begin{figure}[tbp]
%   %\vspace{-3mm}
%   \centering
%   \includegraphics[width=0.45\textwidth]{polyshard_updated_figure.pdf}
%   \vspace{-4mm}\caption{Blockchain, conventional sharding and \tt{Polyshard}.  }
%   \label{fig:sharding}
%   %\vspace{-7mm}
% \end{figure}

% \begin{figure}
% \centering
%     \subfigure[Full replication. 3 blocks verified per epoch. Can tolerate $\frac{N}{2}-1=14$ malicious nodes.]{\includegraphics[width=0.43\linewidth]{figures/full_replication.png}}\hspace{10pt}
%     \subfigure[Sharding with 3 shards. 9 blocks verified per epoch. Can tolerate $\frac{N}{2K}-1=4$ malicious nodes.]{\includegraphics[width=0.5\linewidth]{figures/sharding.png}}
%     \caption{A blockchain system with 30 nodes, each of which is capable of verifying 3 transactions per epoch. With 3-sharding, the ledger is partitioned into 3 sub-ledgers, and transactions are limited to between the accounts within the same sub-ledger. Sharding improves the storage and throughput efficiency by 3 time, at the cost of compromising security by about 3 times.}
%     \label{fig:fr_and_sharding}
% \end{figure}

\begin{figure}[t]
\centering
    \includegraphics[width=0.75\linewidth]{figures/polyshard.png}
    \caption{The proposed {\tt PolyShard} system with 30 nodes. Each node computes a verification function on a coded sub-ledger and a coded block, which are created by a distinct linear combination of the original sub-ledgers, and the proposed blocks respectively. Since encoding does not change the size of the sub-ledger, {\tt PolyShard} achieves the same storage and throughput efficiency (i.e., 9 transactions per epoch) as the conventional sharding solution. Additionally, {\tt PolyShard} improves the security guarantee to protect against $(N-K)/2=13$ malicious nodes, for degree-$1$ verification functions.}
    \label{fig:polyshard}
    \vspace{-3mm}
\end{figure}

% {\bf The illustration in Figure~\ref{fig:sharding} compares and contrasts {\tt Polyshard},  sharding and regular storage approaches in blockchains. The dark circles correspond to nodes, above which the stored blockchain is shown. The different colors in the second row correspond to distinct shards, and {\tt Polyshard} mixes the shards (colors).}

While  coding  is generally applicable in many distributed computing scenarios, the following two salient features make {\tt PolyShard} particularly suitable for blockchain systems.
\begin{itemize}[leftmargin=*]
    \item {\em Oblivious}: The coding strategy applied to generate coded shards is oblivious of the verification function. That means, the same coded data can be simultaneously used for multiple verification items (examples: digital signature verification and balance checking in a payment system);
    \item {\em Incremental}: {\tt PolyShard} allows each node to grow its local coded shard by coding over the newest verified blocks, without needing to access the previous ones. This helps to maintain a constant coding overhead as the chain grows.  
\end{itemize}

%As a proof of concept, we  simulate a payment blockchain system, which keeps records of balance transfers between accounts, and verifies new blocks by checking the senders' fund sufficiency. %We simulate this system for up to $t=1000$ epochs, under various network size $N$ ranging from $15$ to $150$ nodes. 
%We run experiments on this system for various combinations of network size and chain length, and measure/evaluate the throughput, storage, and security achieved by the full replication, sharding, and the {\tt PolyShard} schemes. As we can see from the measurements plotted in Figure~\ref{fig:thpt_N_intro}, {\tt PolyShard} indeed achieves the throughput scaling with network size as the uncoded sharding scheme, improving significantly over the full replication scheme. These experiments provide an empirical  verification of the theoretical guarantees of   {\tt PolyShard} in simultaneously scaling storage efficiency, security, and throughput.

%\begin{figure}[htbp]
%\vspace{-4mm}
%\setlength{\abovecaptionskip}{-0.2em}
%\setlength{\belowcaptionskip}{-1em} 
  %\centering
  %\includegraphics[width=0.5\textwidth]{./figures/thpt_N.png}
  %\caption{Measured throughput of verification schemes; here  number of epochs $t=$1000.}
  %\vspace{-3mm}
  %\label{fig:thpt_N_intro}
%\end{figure}

% \textbf{Songze and Fisher: please expand this section, describing the simulations/experiments. It would be good to also bring a figure on the throughput scaling here.}



\noindent{\bf Other related works.} 
% As mentioned earlier, sharding is the state-of-the-art approach to scale the computation, communication, and storage of blockchain systems
Prominent sharding proposals  in the literature are  \cite{luu2016secure,kokoris2017omniledger,gencer2017short,gao2017proof,zamanirapidchain,bano2017road,ren2018scale,yoo2018blockchain,cai2018decentralized,chauhan2018blockchain,manshaei2018game,EthereumSharding,gencer2016service,al2017chainspace,forestier2018blockclique}.
% The key idea is to partition the entire blockchain into $K$ shards, each of which is managed by a disjoint subset of nodes (miners). This reduces the required amount of computation by a factor of $K$.
As an example, {\tt ELASTICO} \cite{luu2016secure} partitions the   incoming transactions into shards, and each shard is verified by a  disjoint committee of nodes in parallel.  {\tt OmniLedger}~\cite{kokoris2017omniledger} improved upon {\tt ELASTICO} in multiple avenues, including new methods to assign nodes into shards with a higher security guarantee, an atomic protocol for cross-shard transactions, and further optimization on the communication and storage designs.
% For all current sharding systems, in order to scale out with the number of nodes $N$, the number of shards $K$ needs to grow with $N$, i.e., $K = O(N)$. This results in a constant number of nodes in each shards, which makes the system more susceptible to adversaries as the network expands. Current systems achieve security through system solutions such as  shard rotation~\cite{luu2016secure,kokoris2017omniledger,zilliqa}.
% For example, {\tt OmniLedger} leverages {\tt RandHound}~\cite{syta2017scalable}, a bias-resistant distributed randomness generation protocol, to randomly sampling the subset of users assigned to a shard, and randomly updating the these subsets regularly over time. Such methods can provide near-optimal security when the adversarial nodes are fixed prior to the random assignment, but are susceptible when the adversary is dynamic and can corrupt nodes {\em after} they have been assigned to the shards.

==> ISIT/2-ISIT-formulation.tex <==
\vspace{-2mm}
\section{Problem Formulation: Block Verification}
A blockchain system manages a decentralized ledger of its clients' transactions, over a large number of untrusted network nodes. The clients submit their transactions to the network nodes, who group the transactions into blocks that to be included in the system. The accepted blocks are organized into a chain where each block contains a hash pointer to its predecessor. The chain structure provides high security guarantee since for an adversary to tamper the contents of any block, it has to re-grow the entire chain afterwards, which is extremely expensive in computation power. Here we consider a \emph{sharded} blockchain system whose grand ledger is partitioned into $K$ independent shards, each of which maintains a disjoint sub-chain that records the transactions between the accounts associated with the same shard. \footnote{We focus on transactions that are verifiable intra-shard for the sake of clarity. Extensions such as cross-shard transactions and their verification is an added complexity yet complementary to the contributions of this paper. For instance, the atomic payment and locking mechanisms of \cite{kokoris2017omniledger} can be naturally incorporated with the ideas in this paper.}
At a high level, at each time epoch, every shard proposes one block of transactions, and verifies it over the current state of its sub-chain. Once the block passes the verification, it will be appended to the corresponding sub-chain. We now define the system formally.%in more details.
\vspace{-2mm}
\subsection{Computation model}
Each shard $k$ ($k\in[1, K]$) maintains its own sub-chain. We denote the state of the $k$-th sub-chain before epoch $t$ by $Y^{t-1}_{k}=(Y_k(1),\ldots, Y_k(t-1))$, where $Y_k(t) \in \mathbb{U}$ denotes the block accepted to shard $k$ at epoch $t$, and $\mathbb{U}$ is a vector space over a field $\mathbb{F}$. When a new block $X_k(t) \in \mathbb{U}$ is proposed for shard $k$ in epoch $t$ (using some consensus algorithm like proof-of-work (PoW)), the blockchain system needs to verify its legitimacy (e.g., sender accounts have sufficient fund, no double-spending) over the current state $Y^{t-1}_{k}$. %and then reach a consensus on whether to accept it as $Y_k(t)$ or not.
We abstract out the mechanism which generates the proposals and focus on verifying the proposed blocks.
% We note that the proposal can be generated by a small number of nodes, while security depends on the number of nodes that validates the transactions.
% Note that since transactions are intra-shard, the sub-chain is sufficient to verify whether $X_k(t)$ is valid. 

We denote the verification function by $f^t: \mathbb{U}^t \rightarrow \mathbb{V}$, over $X_k(t)$ and the sub-chain $Y_k^{t-1}$, for some vector space $\mathbb{V}$ over $\mathbb{F}$. For instance, for a cryptocurrency blockchain that keeps records of balance transfers between accounts (e.g., Bitcoin), typical verification functions include %the following verification functions are computed to confirm the validity of the payment transactions.  
\begin{itemize}[leftmargin=*]
    \item \emph{Balance checking}: to check each transaction has more input values than those spent in its outputs; and also check that the transactions in a block contain sufficient funds to pay the transaction fees/mining rewards.
    % to check whether the senders have sufficient funds to cover the transactions and the fees/mining rewards;
    % For instance, check each transaction has more input values than those spent in its outputs; and also check that the transactions in a block contain sufficient funds to pay the transaction fees/mining rewards to the block miners.
    \item  \emph{Signature checking}: to verify that a payment transaction spending some funds in an account is indeed submitted by the owner of that account. This often involves computing cryptographic hashes using the account's public key, and verifying the results with the digital signature.
    % \emph{Cryptographic hashing}: to compute the hash of certain inputs, which plays a central role for security, such as malicious miner detection (through PoW and Merkle root verification) and UTXO collection authorization (through digital signature verificaiton).
    % to detect malicious miners by verifying the PoW and the Merkle hash. It is also the core operation for digital signature verification with which input accounts are authorized to collect the output values from previous blocks. 
\end{itemize}
Having obtained $h_{k}^t = f^t(X_k(t), Y_k^{t-1})$, shard~$k$ computes an indicator variable $e_k^t\triangleq\mathbbm{1}(h_k^t \in \mathcal{W})$,
% \begin{align}
%     z_k^t = \mathbbm{1}(h_k^t \in {\cal W}),
% \end{align}
% The value of the variable $z_k^t$ indicates whether the block $X_k(t)$ is valid or not.
where $\mathcal{W} \subseteq \mathbb{V}$ denotes the set of function outputs that affirm $X_k(t)$.
% A simple example is when $\mathbb{V} = \{0,1\}$, the output is binary and denotes the validity, i.e., $\mathcal{W} = \{1\}$. [Fisher: this example is confusing and does not provide much information. Why W=1? Why can't W=0?] 
Finally, the verified block $Y_k(t)$ is computed as $Y_k(t) = e_k^t X_k(t)$, and added to the sub-chain of shard $k$. We note that if the block is invalid, an all-zero block will be added at epoch $t$.

% Without loss of generality, we model the verification function $f^t$ as a multivariate polynomial of degree $d$, motivated by the following result \cite{zou2011representing}:  Any Boolean function $\{0,1\}^n \rightarrow \{0,1\}$ can be represented by a polynomial of degree $\leq n$ with at most $2^{n-1}$ terms. 
% Due to this result, common verification functions, such as balance check and digital signature verification, can all be transformed into polynomials; details are available in Appendix~\ref{sec:field}. 

% \begin{align}\label{eq:verified_block}
%     Y_k(t) = z_k^t X_k(t).
% \end{align}

% \begin{itemize}
%     \item The degree of $f^t$ is determined by the type of verification performed on the block (e.g., computing the current account balance of the sender in a block), and is a fixed constant for a particular type of verification.
%     \item  The number of terms in $f^t$ is proportional to the length of the sub-chain, i.e., $t$. Therefore, the complexity of computing $f^t$ is $O(t)$.
% \end{itemize}

% , for $L$ past blocks used for verification, and some constant $U$ denoting the output size, is a multi-variant polynomial with vector coefficients, and its degree, denoted by $\deg(f_k^t)$, is a constant independent of the input size $L$. As an example, $f_k^t(X_i^{t-1})$ computes the total balance of the client in the block $X_k(t)$ available in shard~$i$ by summing up all the block balances for this client in $X_i^{t-1}$. Also, we assume that the computation complexity of $f_{k}^t$ scales linearly with its input size $L$. Hence, verifying a block over a single shard is
% $K$ times less expensive compared with verification over the entire blockchain.

% \noindent {\bf Example: a payment system.}
% \begin{example}[Balance verification]\label{ex:payment}
% We consider a simple payment blockchain system that keeps records of the balance transfers between clients. We assume that there are $M$ clients in each shard, for some constant $M$ that does not scale with $t$. In this scenario, a block submitted to shard $k$ at time $t$, $X_k(t)$, consists of multiple transactions, and is represented by a pair of real vectors $X_k(t) = (X_k^{\textup{send}}(t), X_k^{\textup{receive}}(t))$, for some $X_k^{\textup{send}}(t), X_k^{\textup{receive}}(t) \in \mathbb{R}^M$. A transaction that reads ``Client $p$ sends $s$ dollars to client $q$.'' will deduct $s$ from $X_k^{\textup{send}}(t)[p]$ and add $s$ to $X_k^{\textup{receive}}(t)[q]$. Clients that do no send/receive money will have their entries in the send/receive vectors set to zeros. To verify $X_k(t)$, we need to check that all the senders in $X_k(t)$ have accumulated enough unspent funds from previous transactions. This naturally leads to the following verification function.
% %where $X_k^{\textup{send}}(t)$ has negative entries and represents the amount of money spent by the clients in shard $k$, and $X_k^{\textup{receive}}(t)$ has positive entries and represents the amount of money received by the clients in shard $k$. In this case, the verification function becomes
% \begin{align}
%      f^t(X_k(t), Y_k^{t-1}) = X_k^{\textup{send}}(t) + \sum_{i=1}^{t-1} (Y_k^{\textup{send}}(i) +Y_k^{\textup{receive}}(i)). \label{eq:multiTrans_verify}
% \end{align}


% Here  the verification polynomial $f^t$ has constant degree $d=1$, with $\mathbb{F}=\mathbb{R}$, $\mathbb{U} = \mathbb{R}^M$, and $\mathbb{V} = \mathbb{R}^M$. We claim the block $X_k(t)$ valid if none of the entries of the above verification function is negative, and we set $Y_k(t) = X_k(t)$ and append it the sub-chain of shard $k$. Otherwise, we append a dummy all-zero block. 

% a block submitted to shard $k$ at time $t$, $X_k(t)$, contains a single transaction that is represented as a real vector of length $M$, i.e., $X_k(t) \in \mathbb{R}^M$. Each block records a balance transfer between a pair of clients.%\footnote{We assume that each client sends or receives at most one payment in each block.} 
% That is, if client $p$ sends $s$ dollars to client $q$ in shard $k$ at time $t$, then $X_k(t)$ will have 
% \begin{align}
%   X_k(t)[i] =  \begin{cases}
%     -s, & i=p\\
%     s, & i=q\\
%     0, & \mathrm{otherwise}
%     \end{cases}.
% \end{align}
% To verify if the above block is valid or not, one simply sums up all the past verified blocks $Y_k(1),Y_k(2),\ldots,Y_k(t-1)$ with $X_k(t)$, and claims that $X_k(t)$ is valid if none of the elements in the sum is negative, and invalid otherwise. More precisely, the function $f^t(X_k(t), Y_k^{t-1})$, $k=1,2,\ldots,K$, is
% \begin{align}
%     f^t(X_k(t), Y_k^{t-1}) = X_k(t) + Y_k(t-1) + \cdots + Y_k(1). 
% \end{align}

% When each block contains multiple transactions initiated from distinct clients, we can represent each block using a pair of real vectors $X_k(t) = (X_k^{\textup{send}}(t), X_k^{\textup{receive}}(t))$, where $X_k^{\textup{send}}(t)$ has negative entries and represents the amount of money spent by the clients in shard $k$, and $X_k^{\textup{receive}}(t)$ has positive entries and represents the amount of money received by the clients in shard $k$. In this case, the verification function becomes
% \begin{align}
%      f^t(X_k(t), Y_k^{t-1}) = X_k^{\textup{send}}(t) + \sum_{i=1}^{t-1} (Y_k^{\textup{send}}(i) +Y_k^{\textup{receive}}(i)). \label{eq:multiTrans_verify}
% \end{align}
% \begin{align}
%      f^t(X_k(t), Y_k^{t-1}) = X_k^{\textup{send}}(t) + Y_k^{\textup{send}}(t-1) +Y_k^{\textup{receive}}(t-1) + \cdots + Y_k^{\textup{send}}(1) +Y_k^{\textup{receive}}(1). \label{eq:multiTrans_verify}
% \end{align}


% {\color{red}[Fisher: The reviewer might criticize why not reduce the verification complexity to a constant by storing the balance. I guess we store the transactions mainly for recurrence? Then we should highlight this.]}

% {\color{blue}[Songze: It is also fine to store the balance, with the difference that the coded chain at each node will not grow with time. Also, as discussed in scenario 3 in Section~\ref{sec:performance}, we lost throughput scaling for constant verification complexity.]}
%\end{example}

% \begin{example}[Arbitrary Boolean functions]\label{ex:arbitrary}
% For blockchain systems that verify incoming blocks based on the most recent $P$ verified blocks, for some constant $P$ (e.g., a payment system that keeps records of clients' account balances and updates the records every $P$ transactions), we can generally model each incoming block $X_k(t)$, and each verified block $Y_k(j)$ as a binary bit stream of length $T$, i.e., $\mathbb{U} = \{0,1\}^T$, and the verification function $f^t: \{0,1\}^{T(P+1)} \rightarrow \{0,1\}$ as a Boolean function that indicates whether $X_k(t)$ is valid or not. According to~\cite[Theorem 2]{zou2011representing}, any arbitrary Boolean function $f$ whose inputs are $d$ binary variables can be represented as a multivariate polynomial $p$ of degree $d$ as follows. For each vector $\vct{a} = (a_1,\ldots,a_d) \in \{0,1\}^d$, we define $h_{\vct{a}} = z_1z_2\cdots z_d$, where $z_i = x_i$ if $a_i=1$, and $z_i=y_i$ if $a_i=0$. Next, we partition $\{0,1\}^T$ into two disjoint subsets $S_0$ and $S_1$ as follows.
% \begin{align}
%     S_0 &= \{\vct{a} \in \{0,1\}^T, f(\vct{a}) =0\},\\
%     S_1 &= \{\vct{a} \in \{0,1\}^T, f(\vct{a}) =1\}.
% \end{align}
% The polynomial $p$ is then constructed as 
% \begin{align}
%     p(x_1,\ldots,x_d, y_1,\ldots,y_d) = \sum_{\vct{a} \in S_1} h_{\vct{a}} = 1 + \sum_{\vct{a} \in S_0} h_{\vct{a}}.\label{eq:boolPoly}
% \end{align}
% Using this transformation, we can represent the verification function $f^t$ with $T(P+1)$ bits input as a multivariate verification polynomial $p^t$ of degree $T(P+1)$ with at most $2^{T(P+1)-1}$ terms. %In this case, the computational complexity $c^t = O(t2^t)$

% We note that this model applies to verifying the digital signatures in the incoming blocks, where the verification does not depend on past blocks, i.e., $P=0$. Utilizing the above technique, we can transfer the required non-polynomial computations like inversions and hash functions over some large prime field into polynomial evaluations.
% \end{example}

% \noindent {\bf Model 2: blocks contain clients' IDs.} In this model, a block $X_k(t)$ contains two elements $X_k(t)[1], X_k(t)[2] \in \mathbb{F}_{2^m}$, which denote the IDs of the sender and the receiver, and $m = \log M$ is the number of bits needed to represent the ID of a client. Then, a block $X_k(t)$ reads ``client $X_k(t)[1]$ in shard $k$ sends one dollar to client $X_k(t)[2]$ in shard $k$ at time $t$''. In this case, $X_k(t)$ is valid if the sender has at least one dollar in its account. Therefore, the verification function computes the account balance of the sender till time $t-1$, i.e., 
% \begin{align}
%   f^t(X_k(t), Y_k^{t-1}) = \sum_{j=1}^{t-1} \mathbbm{1}(X_k(t)[1]=Y_k(j)[2])-\mathbbm{1}(X_k(t)[1]=Y_k(j)[1]).
% \end{align}
% {\bf Goal: model the above indicator function as a polynomial of $X_k(j)[i]$. We know that it can be modelled as a polynomial of degree $2m$ with $2^{2m-1} = M^2/2$ terms for binary indicator functions.}
\vspace{-3mm}
\subsection{Networking model}
The above blockchain system is implemented distributedly over $N$ untrusted nodes. We consider a homogeneous and synchronous network, i.e., all nodes have similar process power, and the delay of communication between any pair of nodes is bounded by some known constant. A subset $\mathcal{M} \subset \{1,\ldots,N\}$ of the nodes may be corrupted, and are subject to Byzantine faults, i.e., they may compute and communicate arbitrary erroneous results during block verification. We aim to design secure verification schemes against the following strong adversary model:
\begin{itemize}[leftmargin=*]
    \item The adversaries can corrupt a fixed fraction of the network node, i.e., the number of malicious nodes grows linearly with $N$.\footnote{While here the adversary model is defined in a permissioned setting, the model and the proposed solution can directly extend to a permissionless setting where e.g., in a PoW system, the adversaries can control a fixed fraction of the entire hashing power.}
    \item If a conventional sharding solution were employed, the adversaries know the allocation of nodes to the shards, and are able to adaptively select the subset $M$ of nodes to attack.
\end{itemize}
We note that under this adversary model, the random shard rotation approach~\cite{luu2016secure,kokoris2017omniledger} is no longer secure since the adversaries can focus their power to attack a single shard after knowing which nodes are assigned into this shard. 
% nodes. We consider an adaptive adversary model, namely, the adversaries know the allocation of nodes to the shards, and are able to selectively attack any $M$ out of the $N$ nodes. The set of nodes under attack is denoted by $\mathcal{M} \subset \{1,\ldots,N\}$. They become malicious and are subject to Byzantine faults, i.e., they may compute and communicate arbitrary erroneous results during block verification. 
Next, we present the networking protocol that will be followed by the honest nodes. Note that adversarial nodes are not required to follow this protocol.%We present next the networking protocol, which will only be followed by the honest nodes.
% A subset $\mathcal{M} \subset \{1,\ldots,N\}$ of these nodes may be malicious/adversarial and subject to Byzantine faults, i.e., they may compute and communicate arbitrarily erroneous results during the block verification process. [I removed this part because the nodes cannot be born to be malicious. Such fixed malicious pattern can be solved by shuffling. For our model to make sense, nodes must be dynamically attacked and become malicious.]
% Furthermore, we consider the class of quickly-adaptive adversaries that can attack the nodes after they are assigned to a particular shard, which renders the random shard rotation approach~\cite{luu2016secure,kokoris2017omniledger} of little effect in protecting the system. Next, we present the networking protocol that will only be followed by the honest nodes.
% [Fishe: It is odd and too defensive to analyze the security performance of shuffling in this section. We should discuss this in Section 3 where we analyze the performance of uncoded sharding.]
% a maximum $\mu$ ($0 \leq \mu \leq \frac{1}{3}$) fraction of them may be malicious, and may 
%compute return arbitrarily erroneous results when queried for block verification. %\footnote{We note that $ \frac{1}{3}N$ is the maximum number of Byzantine failures a practical system with $N$ network nodes can tolerate~\cite{castro1999practical}.}

\noindent {\bf Storage.} At epoch $t$, each node $i$, $i=1,\ldots,N$, locally stores some data, denoted by $Z_i^{t-1} = (Z_i(1),\ldots,Z_i(t-1))$, where $Z_i(j) \in \mathbb{W}$ for some vector space $\mathbb{W}$ over $\mathbb{F}$. The locally stored data $Z_i^{t-1}$ is generated from all shards of the blockchain using some function $\phi_i^{t-1}$, i.e., $Z_i^{t-1} = \phi_i^{t-1}(Y_1^{t-1},\ldots,Y_K^{t-1})$.
% \begin{align}
%     Z_i^{t-1} = \phi_i^{t-1}(Y_1^{t-1},Y_2^{t-1},\ldots,Y_K^{t-1}).
% \end{align}

\noindent {\bf Verification.} Given the $K$ proposed blocks $\{X_k(t)\}_{k=1}^K$, one for each shard, the goal of block verification is to compute $\{f^t(X_k(t),Y_k^{t-1}\}_{k=1}^K$ distributedly over untrusted nodes. We implement this verification process in two steps. In the first step, each node $i$ computes an intermediate result $g_i^t$ using some function $\rho_i^t$ on the proposed blocks and its local storage, such that $g_i^t = \rho_i^t(X_1(t),\ldots,X_K(t),Z_i^{t-1})$,
% \begin{align}
%     g_i^t = \rho_i^t(X_1(t),X_2(t),\ldots,X_K(t),Z_i^{t-1}),
% \end{align}
and then broadcasts the result $g_i^t$ to all other nodes. %{\color{red}[Fisher: Shouldn't we also encode the blocks, whilst keep the verification function $f^t$ unaltered?]} 
%We assume a synchronous network, so that each node will receive all broadcast messages within a constant delay.

The nodes exploit the received computation results to reduce the final verification results in the second step. Specifically, each node $i$ decodes the verification results for all $K$ shards $\hat{h}^t_{1i},\ldots,\hat{h}^t_{Ki}$, 
% Then, the verification results $z_1^t,z_2^t,\ldots,z_K^t$ are decoded from the local computation results of all $N$ nodes, 
using some function $\psi_i^t$, i.e., $    (\hat{h}^t_{1i},\ldots,\hat{h}^t_{Ki})= \psi_i^t(g_1^t,\ldots,g_N^t)$. 
% \begin{align}
%     (\hat{h}^t_{1i},\hat{h}^t_{2i},\ldots,\hat{h}^t_{Ki})= \psi_i^t(g_1^t,g_2^t,\ldots,g_N^t).
% \end{align}
Using these decoded results, node $i$ computes the indicator variables $\hat{e}_{ki} = \mathbbm{1}(\hat{h}_{ki} \in \mathcal{W})$, and then the verified blocks $\hat{Y}_{ki}(t) = \hat{e}^t_{ki}X_k(t)$, for all $k=1,\ldots,K$. Finally, each node~$i$ utilizes the verified blocks to update its local storage using some function $\chi_i^t$, i.e., $ Z_i^t =  \chi_i^t(\hat{Y}_{1i}(t),\ldots,\hat{Y}_{Ki}(t), Z_i^{t-1}) = \phi_i^t(\hat{Y}_{1i}^t,\ldots, \hat{Y}_{Ki}^t)$. Here $\hat{Y}_{ki}^t$ is the sequence of blocks in shard $k$ verified at node~$i$ up to time $t$. To update the local storage $Z_i^t$, while node~$i$ can always apply $\phi_i^t$ on the uncoded shards $\hat{Y}_{1i}^t,\ldots, \hat{Y}_{Ki}^t$, it is highly desirable for $\chi_i^t$ to be {\em incremental}: we only need to create a coded block from $\hat{Y}_{1i}(t),\ldots,\hat{Y}_{Ki}(t)$, and append it to $Z_i^{t-1}$. This helps to significantly reduce the compational and storage complexities. 
% appends the verified block $\hat{Y}_{ki}(t)$ onto the sub-chain $Y_k^{t-1}$ to obtain $\hat{Y}_{ki}^t = (Y_k^{t-1},\hat{Y}_{ki}(t))$, for all $k=1,2,\ldots,K$,  and updates the local storage as follows.
% the $K$ verified blocks are computed as in~(\ref{eq:verified_block}), and appended to the sub-chains at the $K$ shards to obtain $Y_1^t,Y_2^t,\ldots,Y_K^t$, and the storage at node~$i$, $i=1,2,\ldots,N$ is updated as 
% \begin{align}
%     Z_i^t =  \chi_i^t(\hat{Y}_{1i}(t),\hat{Y}_{2i}(t),\ldots,\hat{Y}_{Ki}(t), Z_i^{t-1}).
% \end{align}

\subsection{Performance metrics}
We denote a block verification scheme by $S$, defined as a sequence of collections of the functions, i.e., $S = (\{\phi_i^t,\rho_i^t, \psi_i^t,\chi_i^t\}_{i=1}^N)_{i=1}^{\infty}$. We are interested in the following three performance metrics of $S$.
% \begin{definition}[Storage capacity]
% We define the storage capacity, denoted by $S$, as the average amount of data stored per network node, normalized by the size of the entire block chain, i.e.,
% \begin{align}
%     S = \limsup_{t \rightarrow \infty} \frac{\sum_{i=1}^N size(Z_i^t)}{N\sum_{k=1}^K size(Y_k^t)}. \textup{   {\bf Or use entropy instead of size.}}
% \end{align}
% \end{definition}

\noindent {\bf Storage efficiency}. 
Denoted by $\gamma_S$, it is defined as the ratio between the size of the entire block chain and the size of the data stored at each node, i.e.,
\begin{align}
    \gamma_S \triangleq \frac{K \log |\mathbb{U}|}{\log |\mathbb{W}|}.
    %\liminf_{t \rightarrow \infty} \frac{\sum_{k=1}^K H(Y_k^t)}{\sum_{i=1}^N H(Z_i^t)/N}. %\textup{   {\bf Or use entropy instead of size.}}
\end{align}
%In other words, it is the normalized chain size over the storage size of each node.

The above definition also applies to a  probabilistic formulation where the blockchain elements $Y_k(j)$s and the storage elements $Z_i(j)$s are modelled as i.i.d. random variables with uniform distribution in their respective fields, where the storage efficiency is defined using the entropy of the random variables.

% \begin{definition}[Computation load]
% We define the computation load, denoted by $C$, as the average (normalized) number of operations in $\mathbb{F}$ performed per network node to correctly verify a block, i.e.,
% \begin{align}
%     C = \limsup_{t \rightarrow \infty} \frac{\textup{total \# of operations to verify $K$ blocks}}{NKc^t}. 
% \end{align}
% We note that the computation load is inversely proportional to the throughput of the system.
% \end{definition}

\noindent {\bf Security.}  We say $S$ is $b$-secure if the honest nodes can recover all the correct verification results under the presence of up to $b$ malicious nodes. More precisely, for any subset $\mathcal{M} \subset \{1,\ldots,N\}$ of malicious nodes with $|\mathcal{M}| \leq b$, and each node $i \notin \mathcal{M}$, a $b$-secure scheme will guarantee that $(\hat{h}^t_{1i},\ldots,\hat{h}^t_{Ki}) = (h^t_1,\ldots,h^t_K)$, for all $t=1,2,\ldots$.
% Denoted by $\beta_S$, it is the maximum value of $b$ such that a verification scheme $S$ is $b$-secure.
We define the security of $S$, denoted by $\beta_S$, as the maximum $b$ it could achieve:
\begin{align}
    \beta_S \triangleq \sup\{b: \textup{$S$ is $b$-secure}\}. 
\end{align}
% We note that the computation load is inversely proportional to the throughput of the system.

\noindent {\bf Throughput.} We measure throughput of the system by taking into account the number of blocks verified per epoch and the associated computational cost. We denote by $c(f)$ the computational complexity of a function $f$, which is the number of additions and multiplications performed to evaluate $f$.

We define the throughput of $S$, denoted by $\lambda_S$, as the average number of blocks that are correctly verified per unit discrete round, which includes all the computations performed at all $N$ nodes to verify the incoming $K$ blocks.
% where one verification function $f^t$ with complexity of $c^t$ is computed in a round. 
That is, %{\color{red}[Fisher, you sad throughput is the number of blocks, but the equation seems to be the number of blocks divided by complexity. Should we define throughput as normalized number of blocks per computation operation?]}
\begin{align}
    \lambda_S \triangleq \liminf_{t \rightarrow \infty} \frac{K}{\sum_{i=1}^N (c(\rho_i^t) + c(\psi_i^t) + c(\chi_i^t))/(N c(f^t))}.
    % \liminf_{t \rightarrow \infty} \frac{K}{\textup{total \# of operations to verify $K$ blocks}/(N c^t)}. 
\end{align}
% We note that the computation load is inversely proportional to the throughput of the system.



% {\color{red}[Fisher: Do different techniques have different $c^t$? If yes, then the above normalization may make the comparison unfair, e.g., when the $c^t$ of {\tt PolyShard} is larger than other techniques. It may make sense to remove $c^t$ from the denominator.]}

% {\color{blue}[Songze: $c^t$ is the complexity to compute $f^t$, which does not vary for different techniques.]}

The above three metrics correspond to the three traits in the blockchain trilemma, and all current blockchain systems have to trade off one for another. The goal of this paper is to understand the information-theoretic limits on these metrics, and design verification schemes that can simultaneously achieve the limits, hence settling the trilemma.



==> ISIT/3-ISIT-conventional.tex <==
\vspace{-1.5mm}
\section{Baseline Performance}
\vspace{-1.5mm}
We now present the information-theoretic {\em upper} bounds on the  three performance metrics for any blockchain, and then study the performance of two state-of-the-art blockchain schemes.% and comment on the gaps with respect to the upper bounds.

\noindent {\bf Information-theoretic upper bounds.} 
In terms of security, the maximum number of adversaries any verification scheme can tolerate cannot exceed half of the number of network nodes $N$. Thus, the security $\beta \leq \frac{N}{2}$.
% \begin{align}
%     \beta \leq \frac{N}{2}.
% \end{align}
In terms of storage, for the verification to be successful, the size of the chain should not exceed the aggregated storage resources of the $N$ nodes. Otherwise, the chain cannot be fully stored. We thus have $\gamma \leq N$.
% and this leads to the following upper bound on the storage efficiency.
% \begin{align}
%     \gamma \leq N.
% \end{align}
Finally, to verify the $K$ incoming blocks, the verification function $f^t$ must be executed at least $K$ times in total. Then, we have $\lambda \leq \frac{K}{K/N} = N$.
% \begin{align}
%     \lambda \leq \frac{K}{K/N} = N
% \end{align}
Thus, the information-theoretic upper bounds of security, storage efficiency, and throughput all scale linearly with the network size $N$.

\noindent{\bf Full replication. }
% Using this approach, the local storage and computation are replicated across the entire network. In particular, 
In terms of storage efficiency, since each node stores all the $K$ shards of the entire blockchain, full replication scheme yields $\gamma_{\text{full}}  = 1$.
% \begin{align}
%     \gamma_{\text{full}}  = 1.
% \end{align}
%When a new node joins the network, it has to replicate the entire blockchain into its local storage.
Since every node verifies all the $K$ blocks, the throughput of the full replication scheme is $\lambda_{\text{full}} = \frac{K}{NKc(f^t)/(Nc(f^t))} = 1$. Thus the full replication scheme does not scale with the network size, as both the storage and the throughput remain constant as $N$ increases. The advantage is that the simple majority-rule will allow the correct verification and update of every block as long as there are less than $N/2$ malicious nodes. Thus, $\beta_{\text{full}}=N/2$.
% When receiving the $K$ blocks $X_1(t),\ldots,X_K(t)$ at time $t$, each node computes $K$ verification functions $f^t(X_k(t), Y_k^{t-1})$, $k=1,\ldots,K$. Next, each network node broadcasts its computation results to all the other nodes. For each block, a node decides on its validity using the majority of the received verification results. %i.e., decoding an $(N,1)$ repetition code. 
% This decision will be correct if the number of malicious nodes does not exceed $\frac{1}{2}N$. That is, the full replication scheme has security $\beta_{\text{full}} = \frac{1}{2}N$. After verification, each node appends the verified blocks to their respective sub-chains. The throughput of the full replication scheme $\lambda_{\text{full}} = \frac{K}{NKc(f^t)/(Nc(f^t))} = 1$.

% \begin{align}
%     \beta_{\text{full}} = \frac{1}{2}N.
% \end{align}

%with each other to reach a consensus on the verification results, %using some Byzantine fault-tolerant consensus protocol (e.g., PBFT~\cite{castro1999practical}). 
%After verification, each node appends the verified blocks to their respective sub-chains. %Recall that $f^t$ is a degree-$d$ multivariate polynomial with $\Theta(t)$ terms, hence the complexity for each node to compute $K$ such functions is $O(Kdt)$. 
%The throughput of the full replication scheme $\lambda_{\text{full}} = \frac{K}{NKc(f^t)/(Nc(f^t))} = 1$.
% \begin{align}
%     \lambda_{\text{full}} = \frac{K}{NKc(f^t)/(Nc(f^t))} = 1.
% \end{align}

\noindent{\bf Uncoded sharding scheme.}
In conventional {\em sharding}, the blockchain consists of $K$ disjoint sub-chains known as shards. The $N$ nodes are partitioned into $K$ groups of equal size $q = N/K$, and each group of nodes manage a single shard; this is  a full replication system with $K'=1$ shard and $N'=q$ nodes. 
Since each node stores and verifies a single shard, the storage efficiency and throughput become
$\gamma_{\textup{sharding}} = K$ and $\lambda_{\textup{sharding}} = \frac{K}{Nc^t/(Nc^t)}=K$, respectively. For these two metrics to scale linearly with $N$, it must be true that $K=\Theta(N)$. Consequently, the group size $q$ becomes a constant. Hence, compromising as few as $q/2$ nodes will corrupt one shard and the chain. Thus, this scheme only has a constant security of $\beta_{\text{sharding}}=q/2 =O(1)$. Although system solutions such as shard rotations can help achieve linearly scaling security guarantees, they are only secure when the adversary is non-adaptive (or very slowly adaptive). When the adversary is dynamic, it can corrupt all nodes belonging to a particular shard instantaneously after the shard assignment has been made. Under this model, the security reduces to a constant.  

% \begin{align}
%     \lambda_{\textup{sharding}} = \frac{K}{Nc^t/(Nc^t)}=K$.
% For example, each of the nodes in a group that is responsible for shard~$k$ only stores the sub-chain $Y_k^{t-1}$, and uses it to verify the incoming block $X_k(t)$. Therefore, the uncoded sharding scheme achieves a storage efficiency of $   \gamma_{\textup{sharding}} = \frac{1}{K}$.
% \begin{align}
%     \gamma_{\textup{sharding}} = \frac{1}{K}.
% \end{align}
% On the other hand, to guarantee the correctness of block verification in {\em every} shard, this scheme can tolerate up to $\beta_{\textup{sharding}} = \frac{1}{2}q = \frac{1}{2}\cdot \frac{N}{K}$ malicious nodes.

% the number of malicious nodes cannot exceed $\frac{1}{2}q$. That is, the uncoded sharding scheme has a security of $    \beta_{\textup{sharding}} = \frac{1}{2}q = \frac{1}{2}\cdot \frac{N}{K}$.
% \begin{align}
%     \beta_{\textup{sharding}} = \frac{1}{2}q = \frac{1}{2}\cdot \frac{N}{K}.
% \end{align}

% Since now each node computes one verification function for one shard, the throughput improves by $K$ times over full replication. That is, $    \lambda_{\textup{sharding}} = \frac{K}{Nc^t/(Nc^t)}=K$.
% \begin{align}
%     \lambda_{\textup{sharding}} = \frac{K}{Nc^t/(Nc^t)}=K,
% \end{align}

% The conventional sharding scheme increases the storage capacity and the throughput of the full replication scheme by a factor of $K$. It achieves a linear scaling with the network size $N$ when picking $K = \Theta(N)$.
% The uncoded sharding scheme achieves storage and throughput scaling at the cost of security guarantee. Consider applying the uncoded sharding scheme on a network where the number of malicious nodes increases linearly with the network size (i.e., taking a constant fraction), it will not take long for the malicious nodes to take over one or more shards, and contaminate the entire system. In contrast, for the above full replication scheme, the security $\beta_{\text{full}} = \frac{1}{2}N$ scales linearly with the network size, which continuously enhances the protection against malicious nodes as the network expands.

% The uncoded sharding scheme achieves storage and throughput scaling at the cost of security guarantee. For a network where the number of malicious nodes increases linearly with the network size (i.e., taking a constant fraction), it will not take long for the malicious nodes to take over one or more shards, and contaminate the entire system. 

Neither full replication nor the above sharding scheme exempts from the blockchain trilemma, and has to make tradeoff in scaling towards the information-theoretic limits. 

%Motivated by the recent advances on leveraging coding theory to optimize the performance of distributed computation (see, i.e.,~\cite{li2016fundamental,LMA_all,lee2018speeding,dutta2016short,yu2017polynomial,TLDK-ICML,yu2018lagrangeNIPS}), we propose {\tt PolyShard} (polynomially coded sharding) to achieve all of the three upper bounds simultaneously. Using {\tt PolyShard}, each node stores coded data of the blockchain, and computes verification functions directly on the coded data. %In the following sections, we describe and analyze the {\tt PolyShard} scheme for verifying payment transactions. %From now on, to contrast the conventional sharding scheme from {\tt PolyShard}, we will refer it as ``uncoded sharding''.

% Despite these performance improvements, the sharding scheme is less secure compared with the full replication scheme. In order to achieve linear scaling, we need to maintain the size of a group $N/K$ constant. As the network expands, the number of malicious nodes $\mu N$ becomes larger and larger, and it becomes much easier for them to attack and take over one or more shards. For example, while $\frac{1}{4}N$ malicious nodes cannot compromise a system running the full replication scheme, they can contaminate one of the two shards in a sharding system with $K=2$.



==> ISIT/4-ISIT-balance.tex <==
\vspace{-1mm}
\section{PolyShard for balance checking}\label{sec:balance}
\vspace{-1mm}
In this section, we present {\tt Polyshard} and show how it works on a simple cryptocurrency blockchain system that records  
balance transfers between accounts. We assume that there are $M$ accounts (or addresses) associated with each shard, for some constant $M$ that does not scale with $t$. For the purpose of balance checking, we can compactly represent the block of transactions submitted to shard $k$ at epoch $t$, $X_k(t)$, as a pair of real vectors $X_k(t) = (X_k^{\textup{send}}(t), X_k^{\textup{receive}}(t)) \in \mathbb{R}^M \times \mathbb{R}^M$. %for some $X_k^{\textup{send}}(t), X_k^{\textup{receive}}(t) \in \mathbb{R}^M$. 
Given a transaction in the block that reads ``Account $p$ sends $s$ units to account $q$'', we will have $X_k^{\textup{send}}(t)[p] = -s$, and $X_k^{\textup{receive}}(t)[q] = s$. Accounts that do no send/receive funds will have their entries in the send/receive vectors set to zeros. To verify $X_k(t)$, we need to check that all the sender accounts in $X_k(t)$ have accumulated enough unspent funds from previous transactions. This naturally leads to the following verification function.
%where $X_k^{\textup{send}}(t)$ has negative entries and represents the amount of money spent by the clients in shard $k$, and $X_k^{\textup{receive}}(t)$ has positive entries and represents the amount of money received by the clients in shard $k$. In this case, the verification function becomes
\begin{align}
     f^t(X_k(t), Y_k^{t-1}) = X_k^{\textup{send}}(t) + \sum_{i=1}^{t-1} (Y_k^{\textup{send}}(i) +Y_k^{\textup{receive}}(i)). \nonumber
\end{align}
This function is linear in its input, and has computational complexity $c(f^t) = O(t)$.
%Here  the verification polynomial $f^t$ has constant degree $d=1$, with $\mathbb{F}=\mathbb{R}$, $\mathbb{U} = \mathbb{R}^M$, and $\mathbb{V} = \mathbb{R}^M$. 
We claim the block $X_k(t)$ valid (i.e., $e_k^t=1$) if no entry in the function's output vector is negative, and invalid (i.e., $e_k^t=0$) otherwise. After computation, we have the verified block $Y_k(t) =(Y_k^{\textup{send}}(t), Y_k^{\textup{receive}}(t))=e_k^tX_k(t)$.
%, where $z_k^t$ is the binary variable indicating whether $X_k(t)$ is valid or not.
%and we set $Y_k(t) = X_k(t)$ and append it to the sub-chain of shard $k$. Otherwise, we append a dummy all-zero block. 
Note that this balance checking can be alternatively implemented by having each shard simply store a dimension-$M$ vector that records the aggregated balances of all associated accounts, and the storage and the verification complexity will stay constant as time progresses. However, important transaction statistics including how many transactions occur in each block, and the input/output values in each transaction, and how these statistics evolve over time will be lost in this simplified implementation. Moreover, storing a single block in each shard without the protection of a long chain makes the shard more vulnerable to malicious tampering, compromising the security guarantee. Thus, we stick to the chain structure where all past transactions are kept in the ledger.
% We note that this computation model for balance checking well matches the unspent transaction
% output (UTXO)-based model in practical blockchain systems (e.g., Bitcoin), where a transaction input searches the entire chain for its referenced output from previous transactions that has not been spent. 

We consider operating this sharded payment blockchain %with the above balance checking verification function,
over a network of $N$ nodes, with a maximum $\mu$ fraction of which are corrupted by quickly-adaptive adversaries. For this system, we propose a coded transaction verification scheme, named {\tt PolyShard}, which simultaneously scales the storage efficiency, security, and throughput with the network size. %In what follows, we describe the 
%{\tt PolyShard} consists of three key components: shard encoding, coded verification, and incremental sub-chain update.

\subsection{Coded sub-chain}
In {\tt PolyShard}, at epoch~$t$, each node $i$ stores a coded sub-chain $\tilde{Y}_i^t = (\tilde{Y}_i(1),\ldots,\tilde{Y}_i(t))$ where each component $\tilde{Y}_i(m)$ is a coded block generated by the verified blocks $Y_1(m),\ldots,Y_K(m)$ from all $K$ shards in epoch $m$. The coding is through evaluation of the well-known Lagrange interpolation polynomial. Specifically,  
% are coded blocks 
% blocks generated from blocks in the $K$ shards. In particular, 
we pick $K$ arbitrarily distinct real numbers $\omega_1,\ldots,\omega_K \in \mathbb{R}$, each corresponding to a shard $k$. Then for each $m=1,\ldots, t$, we create a Lagrange polynomial in variable $z$ as follows.
\begin{align}\label{eq:encoding-chain}
    u_m(z) = \sum_{k=1}^K Y_k(m) \prod_{j \neq k} \frac{z - \omega_j}{\omega_k - \omega_j}.
\end{align}
We note that this polynomial is designed such that $u_m(\omega_k) = Y_k(m)$ for all $k=1,\ldots,K$.

Next, , we pick $N$ arbitrarily distinct numbers $\alpha_1,\ldots,\alpha_N \in \mathbb{R}$, one for each node. For each $i=1,\ldots,N$, we create a coded block $\tilde{Y}_i(m)$ that is stored at node~$i$, by evaluating the above $u_m(z)$ at the point $\alpha_i$, i.e.,
\begin{align}
\tilde{Y}_i(m) =  u_m(\alpha_i) = \sum_{k=1}^K Y_k(m) \prod_{j \neq k} \frac{\alpha_i - \omega_j}{\omega_k - \omega_j} = \sum_{k=1}^K \ell_{ik}Y_k(m). \label{eq:hisEncode}
\end{align}
We note that $\tilde{Y}_i(m)$ is a linear combination of the uncoded blocks $Y_1(m),\ldots,Y_K(m)$, and the coefficients $\ell_{ik} = \prod_{j \neq k} \frac{\alpha_i - \omega_j}{\omega_k - \omega_j}$ do not depend on the time index $m$. Therefore, one can think of each node $i$ as having a fixed vector $\ell_{ik}$ by which it mixes the different shards to create $\tilde{Y}_i^t$, and stores it locally.\footnote{The above data encoding is oblivious of the verification function, i.e., the coefficients $\ell_{ik}$ are independent of $f^t$. Therefore, the block encoding of {\tt PolyShard} can be carried out independent of the verification, and the same coded sub-chain can be simultaneously used for all other types of verification items, which could include verifying digital signatures and checking smart contracts.} The size of each coded sub-chain is $K$ times smaller than the size of the entire blockchain, and the storage efficiency of {\tt PolyShard} is  $\gamma_{\textup{{\tt PolyShard}}} = K$.
%\begin{remark}
%The above data encoding is oblivious of the verification function, i.e., the coefficients $\ell_{ik}$ are independent of $f^t$. Therefore, the block encoding of {\tt PolyShard} can be carried out independent of the verification, and the same coded sub-chain can be simultaneously used for all other types of verification items, which could include verifying digital signatures and checking smart contracts.
%\end{remark}

%\begin{figure}[t]
%\vspace{-8mm}
 % \centering
  %\includegraphics[width=0.4\textwidth]{PolyShard.pdf}
  %\caption{Illustration of {\tt PolyShard} scheme.}
 % \vspace{-2mm}
 % \label{fig:PolyShard}
%\end{figure}
\vspace{-2mm}
\subsection{Coded verification}
\vspace{-2mm}
At epoch $t$, each shard $k$ proposes and broadcasts a new block $X_k(t)$ to be added to the sub-chain after balance checking.
%\footnote{This can be done by running some consensus algorithm among a subset of the nodes. Here we omit the description of the consensus phase and focus on verification of the proposed blocks.} %The block $X_k(t)$ can be created by a small group of nodes. For instance as in the uncoded sharding scheme, a subset of $N/K$ nodes run some concensus algorithm to agree on a block to check in each shard. With the $K$ new blocks $X_1(t),\ldots,X_K(t)$ being proposed, they are broadcast through the network for verification. $K$ blocks of transactions $X_1(t),\ldots,X_K(t)$ are created submitted to the $K$ shards for verification. 
%After the new blocks $X_1(t),\ldots,X_K(t)$ are proposed, they are broadcast across the network to all node. 
{\tt PolyShard} verifies these blocks in three steps.
%To start, each of the $K$ incoming blocks is broadcast to all nodes.

\noindent {\bf Step 1: block encoding.} Upon receiving the $K$ proposed blocks, each node~$i$ computes a coded block $\tilde{X}_i(t)$ as a linear combination using the same set of coefficients in (\ref{eq:hisEncode}). That is, $\tilde{X}_i(t) = (\tilde{X}_i^{\textup{send}}(t), \tilde{X}_i^{\textup{receive}}(t))= \sum_{k=1}^K \ell_{ik} X_k(t)$.
% From the $K$ blocks the blockchain system creates a Lagrange polynomial
% \begin{align}
%     u_t(z) = \sum_{k=1}^K X_k(t) \prod_{i \neq k} \frac{z - \beta_i}{\beta_k - \beta_i}.
% \end{align}
% Then, $N$ coded blocks $\tilde{X}_1(t),\tilde{X}_2(t),\ldots,\tilde{X}_N(t)$ are generated as evaluations of the above polynomial at the points $\alpha_1,\alpha_2,\ldots,\alpha_N$, i.e., 
% \begin{align}
%     \tilde{X}_i(t) = u_t(\alpha_i)= \sum_{k=1}^K \ell_{ik} X_k(t).\label{eq:encoding-tran}
% \end{align}
% \begin{align}
%     \tilde{X}_i(t) = \sum_{k=1}^K \ell_{ik} X_k(t).\label{eq:blkEncoding}
% \end{align}
We note that this encoding operation can also be viewed as evaluating the polynomial $v_t(z) = \sum_{k=1}^K X_k(t) \prod_{j \neq k} \frac{z - \omega_j}{\omega_k - \omega_j}$ at the point $\alpha_i$. This step incurs $O(NK)$ operations across the network, since each node computes a linear combination of $K$ blocks.

\noindent {\bf Step 2: coded computation.}
% shard $k$, $k=1,2,\ldots,K$, verifies a block $X_k(t)$ over the $N$ coded shards, using the verification function $f_k^t$. 
Each node $i$ applies the verification function %$f_k^t$, generated from the block $X_k(t)$, for each $k=1,2,\ldots,K$, 
$f^t$ directly to the coded block $\tilde{X}_i(t)$, and its locally stored $\tilde{Y}_i^{t-1}$ to compute an intermediate vector
\begin{align}
g_i^t =  \tilde{X}_i^{\textup{send}}(t) + \sum_{m=1}^{t-1} (\tilde{Y}_i^{\textup{send}}(m) + \tilde{Y}_i^{\textup{receive}}(m)). \label{eq:local_evaluation}
\end{align}
Each node $i$ carries out $\Theta(t)$ operations to compute $g_i^t$, and broadcasts it to all other nodes.
% \begin{align}
%     g_i^t = f^t(\tilde{X}_i(t),\tilde{Y}_i^{t-1}).
% \end{align}

% Since $f^t$ is a degree-$d$ multivariate polynomial with $t$ terms, computing $g_i^t$ has a computational complexity of $O(dt)$, and 
% This step requires a total of $Nc(f^t)$ operations across the network. 

\noindent {\bf Step 3: decoding.}
%Using the computation results $g_1^t,\ldots,g_N^t$, a maximum $\mu$ fraction of which may be erroneous from malicious nodes, each node locally decodes the intended results $\{f^t(X_k(t),Y_k^{t-1})\}_{k=1}^K$. 
It is easy to see that $f^t(v_t(z),u_1(z),\ldots,u_{t-1}(z))$ is a univariate polynomial of degree $K-1$, and $g_i^t$ can be viewed as evaluating this polynomial at $\alpha_i$. Given the evaluations at $N$ distinct points $g_1^t,\ldots,g_N^t$, each node can recover the coefficients of $f^t(v_t(z),u_1(z),\ldots,u_{t-1}(z))$ following the process of decoding a Reed-Solomon code with dimension $K$ and length $N$ (see, e.g.,~\cite{roth2006introduction}). In order for this decoding to be robust to $\mu N$ erroneous results (i.e., achieving security $\beta_{\textup{{\tt PolyShard}}} = \mu N$), we must have $2\mu N \leq N-K$. In other words, a node can successfully decode $f^t(v_t(z),u_1(z),\ldots,u_{t-1}(z))$ only if the number of shards $K$ is upper bounded by $K \leq (1-2\mu)N$. 
% \begin{align}\label{eq:decodability}
%         K \leq \frac{(1-2\mu)N}{d}+1.
% \end{align}
Based on this constraint, we set the number of shards of the {\tt PolyShard} scheme, $K_{\textup{{\tt PolyShard}}} = \lfloor (1-2\mu)N \rfloor$, which scales linearly with network size $N$. The complexity of decoding a length-$N$ Reed-Solomon code at each node is $O(N \log^2 N \log \log N)$, and the total complexity of the decoding step is $O(N^2 \log^2 N \log \log N)$.

Having decoded $f^t(v_t(z),u_1(z),\ldots,u_{t-1}(z))$, each node evaluates it at $\omega_1,\ldots,\omega_K$ to recover $\{f^t(X_k(t),Y_k^{t-1})\}_{k=1}^K$, to obtain the verification results $\{e_k^t\}_{k=1}^K$ and the verified blocks $\{Y_k(t) = e_k^t X_k(t)\}_{k=1}^K$. Finally, each node $i$ computes $\tilde{Y}_i(t)$ following (\ref{eq:hisEncode}), and appends it to its local coded sub-chain.\footnote{The sub-chain update process in {\tt PolyShard} is incremental, i.e., appending a coded block to a coded sub-chain is equivalent to appending uncoded blocks to the uncoded sub-chains, and then encoding from the updated sub-chains. This commutativity between sub-chain growth and shard encoding allows each node to update its local sub-chain incrementally by accessing only the newly verified blocks instead of the entire block history. } Updating the sub-chains has the same computational complexity with the block encoding step, which is $O(NK)$.

% \subsection{Incremental sub-chain update}\label{sec:update}
% The blocks that fail the validation process (i.e., $e_k^t =0$) should be replaced by the zero block in the finalized chain, so we have,  $Y_k(t) = e_k^t X_k(t)$. Each node now calculates
% \begin{align}
%     \tilde{Y}_i(t) = \sum_{k=1}^K \ell_{ik} e_k^t X_k(t)  = \sum_{k=1}^K \ell_{ik}Y_k(t),\label{eq:newEncode}
% \end{align}
% and append $\tilde{Y}_i(t)$ into its local coded sub-chain to update it to $\tilde{Y}_i^t = (\tilde{Y}_i^{t-1}, \tilde{Y}_i(t))$.
% % \begin{align}
% %     \tilde{Y}_i^t = (\tilde{Y}_i^{t-1}, \tilde{Y}_i(t) ). \label{eq:update}
% % \end{align}
%\begin{remark}
%The sub-chain update process in {\tt PolyShard} is incremental, i.e., appending a coded block to a coded sub-chain is equivalent to appending uncoded blocks to the uncoded sub-chains, and then encoding from the updated sub-chains. This commutativity between sub-chain growth and shard encoding allows each node to update its local sub-chain incrementally by accessing only the newly verified blocks instead of the entire block history.  
%\end{remark}

\subsection{Performance of {\tt PolyShard}}\label{sec:performance}
So far, we have shown that {\tt PolyShard} achieves a storage efficiency $\gamma_{\textup{{\tt PolyShard}}} = K_{\textup{{\tt PolyShard}}} = \Theta(N)$, and it is also robust against $\mu N = \Theta(N)$ quickly-adaptive adversaries. The total number of operations during the verification and the sub-chain update processes is
$O(NK) + N\Theta(t) + O(N^2 \log^2 N \log\log N)$, where the term $O(NK) + O(N^2 \log^2 N \log\log N)$ is the additional coding overhead compared with the uncoded sharding scheme. Since $K_{\textup{{\tt PolyShard}}}\leq N$,
% Based on (\ref{eq:decodability}), we pick $K = \lfloor \frac{(1-2\mu)N}{d}\rfloor \leq N$. Therefore, 
the coding overhead %$O(NK) + O(N^2 \log^2 N \log\log N)$
reduces to $O(N^2 \log^2 N \log\log N)$. The throughput of {\tt PolyShard} for balance checking is computed as
\begin{align}
    \lambda_{\textup{{\tt PolyShard}}} &= \liminf_{t \rightarrow \infty} \frac{K_{\textup{{\tt PolyShard}}}N\Theta(t)}{N\Theta(t) + O(N^2 \log^2 N \log\log N)}\\
    &=\liminf_{t \rightarrow \infty} \frac{K_{\textup{{\tt PolyShard}}}}{1 + \frac{O(N\log^2 N \log \log N)}{\Theta(t)}}= \Theta(N). %\label{eq:T_PS}
\end{align}

% Having demonstrated the robustness of {\tt PolyShard} against $\mu N = \Theta(N)$ adversaries, we analyze the storage efficiency and the throughput of {\tt PolyShard}, for the scenario where the verification function $f^t$ has constant degree $d$, and its computation complexity $c(f^t) = O(t)$ scales with the chain length $t$. % in the following scenarios, which correspond to different assumptions on the computational complexity of the verification function $f^t$.
% is decoded with a complexity of $O(N\log^2N \log \log N)$. Finally, each trusted node creates $\frac{N}{K}$ coded blocks with the complexity $O(\frac{N}{K}\cdot K) = O(N)$. Therefore, the throughput of the coded scheme is
% \begin{table}[htbp!]
% \centering % used for centering table
% \caption{Computation complexity breakdowns of block verification schemes} % title of Table
% \begin{tabular}{|c | c | c |c|} % centered columns (4 columns)
% \hline  %inserts double horizontal lines
% \rule{0pt}{15pt}  & Uncoded & Coded, $A$ fixed & Coded, $A = \mu N$\\ [1ex] % inserts table
% %heading
% \hline % inserts single horizontal line
% \rule{0pt}{15pt} \multirow{2}{*}{Encoding} &  & \multirow{2}{*}{$O(N \log^2 N \log \log N)$} & Separate: $O(NK)$\\
% \rule{0pt}{15pt} & & & Proof-certify: $O(N \log^2 N \log \log N)$\\
% [1ex]  % inserting body of the table
% \hline
% \rule{0pt}{15pt} Local computation & $O(NKt)$ & $O(Nt)$ & $O(Nt)$  \\ [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \rule{0pt}{15pt} Decoding & & $O(N \log^2 N \log \log N)$ & Proof-certify: $O(N \log^2 N \log \log N)$ \\ [1ex]
% \hline 
% \rule{0pt}{15pt} \multirow{2}{*}{Recurrent update} & & \multirow{2}{*}{$O(N \log^2 N \log \log N)$} & Separate: $O(NK)$ \\ 
% \rule{0pt}{15pt} & & & Proof-certify: $O(N \log^2 N \log \log N)$\\[1ex]
% \hline
% \end{tabular}
% \label{table:nonlin} % is used to refer this table in the text
% \end{table}
% When $t \gg N$, the overall complexity of the coded scheme is $O(Nt)$, and it is $K$ times less than that of the uncoded scheme.
% \noindent {\bf Scenario 1: the degree $d$ is constant, and the complexity $c(f^t)=O(t)$.} %, and the complexity $c^t = \Theta(t)$.} 
% This is for the verification process that scans through the entire history of the blockchain. For each past block, an operation with fixed complexity is performed (e.g., adding two real vectors for balance checking in Example~\ref{ex:payment}). %The balance verification in Example~\ref{ex:payment} falls into this scenario. %where $c^t = For constant degree $d$, we have $K_{\textup{{\tt PolyShard}}} = \lfloor \frac{(1-2\mu)N}{d}+1 \rfloor = \Theta(N)$, and the storage efficiency $\gamma_{\textup{{\tt PolyShard}}} = \Theta(N)$.
% % \begin{align}
% %     \gamma_{\textup{{\tt PolyShard}}} = \Theta(N).
% % \end{align}

% When $c(f^t) = O(t)$, i.e., the complexity of computing $f^t$ increases with $t$,\Theta(t)$.
% 
% $K = \Theta(N)$, and $N\log^2 N \log \log N = o(c^t)$, 
% the throughput in (\ref{eq:T_PS}) becomes
% \begin{align}
%       \lambda_{\textup{{\tt PolyShard}}} =\liminf_{t \rightarrow \infty} \frac{K_{\textup{{\tt PolyShard}}}}{1 + \frac{O(N\log^2 N \log \log N)}{c(f^t)}}= \Theta(N).
% \end{align}
% This computation load is $\frac{1}{\Theta(N)}$ when $\log^2 N \log\log N = o(t)$, which is almost always true in any practical system. 
% This completes the proof of Theorem~\ref{thm:PolyShard}.

We can see that since the complexities of the encoding and decoding operations of {\tt PolyShard} do not scale with $t$, the coding overhead becomes irrelevant as the chain grows. The {\tt PolyShard} scheme simultaneously achieves information-theoretically optimal scaling on security, storage efficiency, and throughput. We note that when the verification function is linear with the block data, codes designed for distributed storage (see, e.g.,~\cite{dimakis2011survey,rashmi2011optimal}) can be used to achieve similar scaling as {\tt PolyShard}. However, {\tt PolyShard} is designed for a much more general class of verification functions including arbitrary multivariate polynomials, which cannot be handled by state-of-the-art storage codes.

